Read, Look or Listen? What's Needed for Solving a Multimodal Dataset

The prevalence of large-scale multimodal datasets presents unique challenges in assessing dataset quality. We propose a two-step method to analyze multimodal datasets, which leverages a small seed of human annotation to map each multimodal instance to the modalities required to process it. Our method sheds light on the importance of different modalities in datasets, as well as the relationship between them. We apply our approach to TVQA, a video question-answering dataset, and discover that most questions can be answered using a single modality, without a substantial bias towards any specific modality. Moreover, we find that more than 70% of the questions are solvable using several different single-modality strategies, e.g., by either looking at the video or listening to the audio, highlighting the limited integration of multiple modalities in TVQA. We leverage our annotation and analyze the MERLOT Reserve, finding that it struggles with image-based questions compared to text and audio, but also with auditory speaker identification. Based on our observations, we introduce a new test set that necessitates multiple modalities, observing a dramatic drop in model performance. Our methodology provides valuable insights into multimodal datasets and highlights the need for the development of more robust models.

==> sections/checklist.tex <==
\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See \cref{sec:limitations}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{It's in the supplemental material}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See \cref{sec:dataset_experimental_setup}}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerNA{}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See \cref{app:dataset-supp}}
  \item Did you mention the license of the assets?
    \answerYes{See \cref{app:dataset-supp}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{In the supplemental material}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{Everything is done according to the accepted guidelines of Amazon Mechanical Turk.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{We have not gathered any personally identifiable information or offensive content. During the initial annotation phase, we utilized pre-existing questions from the TVQA dataset, which served as our reference. Additionally, when collecting the test set, we thoroughly reviewed and validated its content to ensure the absence of any harmful or objectionable material.}
\end{enumerate}

\item If you used crowd sourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{See \cref{app:workers-analysis} and \cref{app:mmqa}.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerYes{See \cref{app:workers-analysis} and \cref{app:mmqa}.}
\end{enumerate}
\end{enumerate}

==> sections/not_used_AVSD_Analysis.tex <==
We apply our method to the AVSD Audio-Visual Scene-Aware Dialog~\citep{alamri2019audiovisual}.
Below we describe our data collection (\cref{sec:avsd_dataset_experimental_setup}), and how our results provide insights on the AVSD dataset (\cref{sec:avsd_dataset_analysis}).

\subsection{Data Collection}\label{sec:avsd_dataset_experimental_setup}

\newparagraph{AVSD}
The AVSD data set is a comprehensive collection of multimodal data designed for research in audio-visual scene-aware dialog systems. It includes audio recordings, video frames, and textual dialog transcripts, capturing real-world scenarios. 
% The dataset was originally introduced as a  dataset (video frames and subtitles), but we consider \citet{Zellers2022MERLOTRN}'s version, which includes a third modality, namely speech.


\newparagraph{Humans annotations.}
% We hire native English-speaking workers from Amazon Mechanical Turk to answer questions based on a specific modality of the input. We develop qualification tests to select high-quality annotators and divide them into three separate groups, one per modality. Following \citet{Chao2017BeingNB,Wang2021MultiSubsAL}, and \citet{Castro2020LifeQAAR}\netta{check the cites}, we also require participants to answer a yes/no question, indicating whether they think the question can be answered based solely on the specific modality input. However, we find this approach to be less reliable---35\% of the questions marked as unsolvable were, in fact, solvable. As a result, we rely on the annotators accuracy in order to determine whether a question is answerable using a subgroup of modalities, but use the yes/no information for monitoring the quality of their annotations. \footnote{Workers who consistently marked 'yes' or 'no' were excluded, as well as those who showed low agreement with the rest of the group.} 
% Further, to prevent annotators from answering based on memory of already seeing that particular scene, we add a checkbox for them to indicate whether they had seen the scene before, and omit those answers. 

% We select a set of 402 examples from the validation set of AVSD. We break them down to 75\%/15\%/10\% for training/validation/test, respectively. We show each annotator a single modality, and use five annotators for each (instance,modality) combination. The final label is determined based on whether 4 or 5 out of 5 workers answered the question correctly. If this condition is met, the question is marked to be answered using this modality. See \cref{app:avsd-workers-analysis} for more information about the annotation metrics and further analysis.

\newparagraph{Expansion to the full dataset. }
% For each of the TVQA modalities, we train a different classifier, each based on a frozen finetuned \merlot model~\citep{Zellers2022MERLOTRN}, which achieves a relatively high level of accuracy (83\%) on the original TVQA dataset. 
% The classifiers are trained on our human annotated labels,  with balanced class weights for each modality. An illustration of our three classifiers as applied to TVQA is presented in~\cref{fig:third}.
% We conduct a hyperparameter search over the basic parameters of random forest such as the number of trees in the forest, and the maximum depth of each tree. We report test results on the top-performing model on our validation set. See \cref{app:scorer-analysis} for more details.

\newparagraph{Classification results.} 
% \cref{tab:avsd-three_tasks_results} shows our results. Test results range between 74-81\%, on average 12\% higher than a majority baseline. Interestingly, our OOD test results are on par, and sometimes higher than the ID test results, indicating that our annotations generalize to other domains. We also test the effect of the training set size, by training the classifiers with 30\%, 50\% and 70\% of our training data. Our results (\cref{tab:three_tasks_results_different_training_size} in~\cref{app:data-size-analysis}) show that training on as few as 30\% of our original size yields performance comparable to our full training set. This finding not only streamlines the data collection process, but also suggests that strong results can be achieved without further annotation efforts.

\begin{table*}[t]
\caption{\label{tab:avsd-three_tasks_results}
Validation, test accuracy of our classifiers for predicting the solvability of AVSD instances based on a single modality, compared to a majority baseline.
}
\centering
\begin{tabular}{@{}p{0.001cm}p{1.8cm}cccccc@{}} \toprule
\multicolumn{2}{l}{} & 
\multicolumn{2}{c}{Image} & 
\multicolumn{2}{c}{Text} & 
\multicolumn{2}{c}{Audio}  
\\ \cmidrule(l){3-4} \cmidrule(l){5-6} \cmidrule(l){7-8} 
\multicolumn{1}{l}{}   & Approach & Val  & Test   & Val  & Test & Val  & Test \\ \midrule
& Majority             
& \phantom{0} 77              & \phantom{0} 77              & \phantom{0} 57              & \phantom{0} 57        
& \phantom{0} 51              & \phantom{0} 51 \\

& Classifier
& \phantom{0}89              & \phantom{0}81              &\phantom{0} 82              & 
\phantom{0} 74               & 
\phantom{0} 81              &
\phantom{0} 76            \\
                            
\bottomrule
\end{tabular}
\end{table*}

\subsection{Dataset Analysis}\label{sec:avsd_dataset_analysis}
We turn to use our classifiers to analyze the validation set of the AVSD dataset. An analysis based on our seed annotation also yields similar results, see~\cref{app:avsd_analysis_based_on_workers}.

% \begin{figure}[htbp]
% \centering
% \begin{subfigure}[t]{0.48\textwidth}
% % \vspace*{0.5cm}
% \includegraphics[width=\textwidth,scale=2, trim={1cm 0.3cm 1.1cm 0.5cm},clip]{pngs/scorer on all val data hist.pdf}
%     \caption{\label{Histogram val} Proportions of questions answerable using a single modality (top three bars), as well as that of questions unanswerable using any single modality (final bar).}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.48\textwidth}
%     \includegraphics[width=\textwidth,scale=6, trim={4cm 2.5cm 7cm 1cm},clip]{pngs/scorer on all val data venn.pdf}
%         \caption{\label{venn val}
% Each circle in the graph represents a portion of the data answerable using a particular modality. Overlapping areas mark the proportions of instances solvable by either modality separately.}
% \end{subfigure}
% \caption{An analysis of the validation set of the TVQA dataset.}
% \label{fig:validation-splits}
% \end{figure}

\newparagraph{Bias towards the image modality}
% We observe that similar proportions of the questions could be solved by each of the different modalities---63\%/61\%/62\% using image/text/audio, respectively. Prior work~\citep{Winterbottom2020OnMB} used partial-input models and identified a bias towards the text modality in this dataset. Our method, relying on a seed annotation, leads to a different conclusion, and shows no evidence of such bias.

\newparagraph{Almost all questions could be solved using a single modality.}
% \cref{Histogram val} shows the proportions of questions answerable with each modality, as well as the fraction of questions unanswerable using any single modality. Our results confirm previous results~\citep{Winterbottom2020OnMB} and show that almost 99\% of the questions could be solved correctly using a single modality. As a result, we do not further annotate groups of more than one modality.


\newparagraph{Many questions could be solved by more than one modality.}
% The values in~\cref{Histogram val} indicate a large overlap between the instances answerable by the different modalities (as the sum of all bars largely exceeds 100\%).
% To study this overlap, we plot (\cref{venn val}) a Venn diagram, where each circle represents the partitions of instances answerable with a different modality, and overlapped areas represent instances solvable by either modality separately. 
% Our results show that more than 70\% of the instances are solvable using two or more modalities, and more than 15\% using each of the three modalities, further indicating that TVQA instances do not require integration of different modalities.

